Taming Server Memory TCO with Multiple Software-Defined Compressed Tiers

Memory accounts for 33 - 50% of the total cost of ownership (TCO) in modern data centers. We propose a novel solution to tame memory TCO through the novel creation and judicious management of multiple software-defined compressed memory tiers. As opposed to the state-of-the-art solutions that employ a 2-Tier solution, a single compressed tier along with DRAM, we define multiple compressed tiers implemented through a combination of different compression algorithms, memory allocators for compressed objects, and backing media to store compressed objects. These compressed memory tiers represent distinct points in the access latency, data compressibility, and unit memory usage cost spectrum, allowing rich and flexible trade-offs between memory TCO savings and application performance impact. A key advantage with ntier is that it enables aggressive memory TCO saving opportunities by placing warm data in low latency compressed tiers with a reasonable performance impact while simultaneously placing cold data in the best memory TCO saving tiers. We believe our work represents an important server system configuration and optimization capability to achieve the best SLA-aware performance per dollar for applications hosted in production data center environments. We present a comprehensive and rigorous analytical cost model for performance and TCO trade-off based on continuous monitoring of the application's data access profile. Guided by this model, our placement model takes informed actions to dynamically manage the placement and migration of application data across multiple software-defined compressed tiers. On real-world benchmarks, our solution increases memory TCO savings by 22% - 40% percentage points while maintaining performance parity or improves performance by 2% - 10% percentage points while maintaining memory TCO parity compared to state-of-the-art 2-Tier solutions.

==> design.tex <==
\section{Design}
\label{sec:design}

\subsection{Fault distribution}
As noted by others~\cite{hemem} and us, the cover of Intel PEBS is limited to ~10\% to 15\%. This may lead to an incorrect categorization of a hot page as a cold page. Note that, as it never generates false positive events, a cold page can never be marked as a hot page.

We devise a novel way to augment the coverage of hardware counters with the number of faults in different compressed memory tiers. As with the PEBS events, zswap faults are ground truth. There are no false positive or false negative events.

\begin{algorithm}
    \caption{Fault distribution}\label{alg:fault_distribution}
    \begin{algorithmic}

        % \Require $n \geq 0$
        % \Ensure $y = x^n$
        \Require P[(addr, count)] \Comment{PEBS events}
        \Require F[(tier, faults, nr\_regions)] \Comment{Zswap Faults}
        \Require R[(s\_addr, e\_addr, hotness, tier)] \Comment{Regions}
        \For{$\forall r \in R$}  \Comment{For all regions }
        \State $r.hotness=0$
        \For{$\forall p \in P$}
        \If{$r.s\_addr \le p.addr \le r.e\_addr$}
        \State $r.hotness+=p.count$
        \EndIf
        \EndFor
        \State $r.hotness+= \alpha*(F[r.tier].faults/F[r.tier].nr_regions)$
        \EndFor
    \end{algorithmic}
\end{algorithm}




==> future_work.tex <==
\section{Future Work}
\label{sec:future_work}

\subsection{Hints from Faults in a Tier}
The total number of faults recorded serves as a metric of how well our placement policy is. In the ideal case,

\begin{align}
U_0 > U_1  > U_2 > U_3 >  U_4
\end{align}

If we see a higher number of faults for a slow tier, then it clearly indicates that our placement policy made a mistake, and we should immediately begin page promotions from this slow tier to a better tier. The decision of exactly what pages are to be migrated is guided by the region's info collected and built over many profiling time intervals.

\begin{tcolorbox}
In order to promote pages from seeing faults in a particular tier, we need to also maintain the info from which region the faults are coming. All the pages of the responsible region should be promoted.
\end{tcolorbox}


\subsection{Scoring Tiers}
\label{sec:scoring_tiers}

As of now, we are scoring tiers based on the load latency. However, a user might feel difference and might want to rank tiers based on their compressibility or the cost of the storing data on them, or a combination of all the three. 

Here, we define a mathematical model to do so.
\begin{align}
\label{eq:policy}
P: (\alpha, \beta ,\gamma), \text{s.t. } \alpha + \beta + \gamma = 1 \text{ and } \alpha, \beta, \gamma >= 0
\end{align}
Here, $\alpha$ controls the weight of compressibility, i.e., a higher value for $\alpha$ indicates that the higher the compression, better the tier. $\beta$ controls the weight of performance, i.e., the access latency of the tiers. $\gamma$ controls the total TCO.



%We employ the standard min-max and max-min scaling. In the former, the smallest value goes to 0 and the maximum to 1, and in the latter, it's vice-versa. In Equation~\ref{equ:scaling}, $x$ is scaled using min-max scaling, whereas $y$ is scaled using max-min scaling.
%
%\begin{align}
%\label{equ:scaling}
%x\_{sc} = \frac{x-min(X)}{max(X)-min(X)};
%y\_{sc} = \frac{max(Y)-y}{max(Y)-min(Y)} 
%\end{align}

Since in equation~\ref{eq:policy} we are adding terms representing different quantities, the first step is to normalize the values in the different columns in the range of [0,1]. This is a required step in order to combine them into a single value. We scale compressibility, latency, and cost are scaled using max-min scaling. 
%This is because a higher compressibility ratio is desired, whereas, for latency and cost, a lower value is preferred.

\begin{align}
\label{equ:scaling}
%x\_{sc} = \frac{x-min(X)}{max(X)-min(X)};
y\_{sc} = \frac{max(Y)-y}{max(Y)-min(Y)} 
\end{align}

A simple scoring metric can be for a tier $T1$:
\begin{align}
%S^{T1} = \alpha * \compress\_sc_t^{T1} + \beta *\lat\_sc_t^{T1} + \gamma * \usd\_sc_t^{T1}
S_{T1} = \alpha * \compress\_sc_{T1} + \beta *\lat\_sc_{T1} + \gamma * \usd\_sc_{T1}
\end{align}

In a similar manner, we can collect the score of other tiers and then sort them, with the maximum value tier becoming the first, hottest, and fastest tier.

\begin{tcolorbox}
At the moment, in our experiments we will fix the ordering of tiers for a particular workload. The dynamic ordering of tiering is planned for to be implemented in a later version. 
\end{tcolorbox}

\subsection{Modeling migration cost}
Once the mapping of a region to a particular tier is done, the actual migration of the pages can start. However, we need to account for the cost of the migration vs. the benefits of the migration in the future.
Here, we consider the size, the source tier, and the destination tier of a region. We also take into account the faults, size, and pressure on both the source and the destination tiers.

\begin{tcolorbox}
 Migrating a compressed page from one compressed tier to another has some performance implications, especially if the compression algorithm on both of the tiers is different. Here, the only way is to decompress the page using the source compression algorithm and then compress it again with the destination compression algorithm.
\end{tcolorbox}

In order to reduce the cost, the migration daemon can skip some tiers and place it on a tier with the same compression algorithm.


Now, the cost migrating a region ($r_i$) set of pages from one tier to another can be captured using the equation:
\begin{align}
MigCost(r_i,CT_i,DT_i) =  |r|*(D_{CT_i},A_{DT_i},C_{DT_i},Z_{up},PTE_{up})
\end{align}
This gives the cost in terms time taken to complete the operation.

Estimated benefits: The faults that were directed toward the pages being migrated will now be from a better tier.

\begin{align}
Benefit_{mig\_r_i} = (\lat(CT_i) - \lat(DT_i))*Exp(Faults_{r_i})
\end{align}

We only migrate when the benefits or migrating a region is higher the cost of doing so.

%\subsection{When to do migration?}
%
%\textbf{When to do demotions?}
%What is the cost of keeping them in the current tier? And is it justified? How to analytically answer this question if they are justified or not?
%Ans: If the faults in the region are within a threshold. 
%\begin{tcolorbox}
%Every tier must have a range for total faults associated with it based on its size (faults/size ?). If the number of faults within this region is within this number, then it provides a good balance between the TCO savings and the performance loss. For example, for a TB size region, we must see total accesses to be within $X$ and $Y$.
%\end{tcolorbox}



==> learnings.tex <==
\section{Learnings}
\label{sec:learnings}

\subsection{N-Tier is paving the way for future memory solutions}
TODO
\subsection{Advancements in Hardware of Compression}
TODO
\subsection{Effective Data movement between Tiers}
TODO

\subsection{Aggression in Data Movement}
\label{sec:aggression_data_movemet}

In a TCO saving scheme, applying a policy to decide on the placement of data pages is the first step. The second step is to move the data to their destination tiers.
Depending on the amount of data movement, this step may take a while.
Ideally, we want all the data movement to finish during a profile window so that when the profile window ends, we have a fresh set of data pages and corresponding tiers, and we start moving data as per this new placement guide.

Since the movement of one data page is independent of another, the movement step can be performed using multiple threads. However, there are implications of using more threads on the application's performance, saved TCO, and the movement tax.

\begin{figure}
    \centering
    \subfloat[Impact on TCO and Performance]{
        \includegraphics[width=.9\linewidth]{FIGS/agg_tco_ops.pdf}
    }
    
    \subfloat[Movement Tax]{
        \includegraphics[width=.7\linewidth]{FIGS/agg_perf.pdf}
    }
\end{figure}


==> pagerank_eval.tex <==

\begin{figure*}
    \centering
    \subfloat[Data placement recommendation by {\methodname}'s waterfall model.]{
    \includegraphics[scale=\scaleval]{FIGS/waterfall_pagerank_regions.pdf}
    }
    \subfloat[Actual tier utilization when using {\methodname}'s waterfall model.]{
    \includegraphics[scale=\scaleval]{FIGS/waterfall_pagerank_pages.pdf}
    }

    \subfloat[Data placement recommendation by {\methodname}'s ILP-30 model.]{
    \includegraphics[scale=\scaleval]{FIGS/ilp_30_pagerank_regions.pdf}
    }
    \subfloat[Actual tier utilization when using {\methodname}'s ILP-30 model.]{
    \includegraphics[scale=\scaleval]{FIGS/ilp_30_pagerank_pages.pdf}
    }

        \subfloat[Tier faults in Google's approach.]{
        \includegraphics[scale=\scalevalsmall]{FIGS/google_pagerank_faults.pdf}
        }
        \subfloat[Tier faults in HEMEM's approach]{
        \includegraphics[scale=\scalevalsmall]{FIGS/hemem_pagerank_faults.pdf}
        }
        
        \subfloat[Tier faults in the {\methodname}'s waterfall model.]{
        \includegraphics[scale=\scalevalsmall]{FIGS/waterfall_pagerank_faults.pdf}
        }
        \subfloat[Tier faults in the {\methodname}'s ILP-30 model.]{
        \includegraphics[scale=\scalevalsmall]{FIGS/ilp_30_pagerank_faults.pdf}
        }
        \subfloat[Tier faults in the {\methodname}'s ILP-90 model.]{
            \includegraphics[scale=\scalevalsmall]{FIGS/ilp_90_pagerank_faults.pdf}
            }
    \caption{Model recommendation and tiers utilization for \memcached.}
\end{figure*}

